Cell-Free Massive MIMO under a Non-Linear Power Amplifier Consumption Model

Existing works on Cell-Free Massive MIMO primarily focus on optimising system throughput and energy efficiency under high-traffic scenarios with only a limited focus on variable user demand as required by higher network layers. Additionally, existing works only minimise the transmitted power instead of the consumed power at the power amplifier. This work introduces a penalty-method-based approach to minimise the amplifier's power consumption while scaling much better with network size than current solutions and promoting sparsity in the power allocated to each access point. Furthermore, we demonstrate substantial reductions in power consumption (up to 24%) by considering the non-linear power consumption.

==> figures/convergence/convergenceSEs.tex <==
\begin{tikzpicture}
\pgfplotstableread[col sep=comma,]{figures/convergence/convergenceSEs.csv}\datatable
\begin{axis}[
    xlabel={Penalty Method Iteration},
    ylabel={Per-user SE [Bps/Hz]},
    legend style={
       at={(0.97,0.05)},
       anchor=south east,
       legend columns=1,
       nodes={scale=0.8, transform shape}},
    grid style={line width=.1pt, draw=gray!10},
    major grid style={line width=.2pt,draw=gray!50},
    grid style=dashed,
    grid=both,
    width=1\linewidth,
    height=0.4\linewidth,
    mark repeat=1,
    xmin=1,
    xmax=10,
]  
  \addplot[style=loosely dashdotted, black!80, domain=1:10, samples=2] {10.5};
  \addlegendentry{Target SE}
   \addplot+[style=solid, mark=+] table [x, y={y1}]{\datatable};
    \addplot+[style=solid, mark=+]  table [x, y={y2}]{\datatable};
         \addplot+[style=solid, mark=+]  table [x, y={y3}]{\datatable};
         \addplot+[style=solid, mark=+] table [x, y={y4}]{\datatable};
         \addplot+[style=solid, mark=+]  table [x, y={y5}]{\datatable};
  \end{axis}
\end{tikzpicture}
